Machine Learning Security in Industry: A Quantitative Survey

Despite the large body of academic work on machine learning security, little is known about the occurrence of attacks on machine learning systems in the wild. In this paper, we report on a quantitative study with 139 industrial practitioners. We analyze attack occurrence and concern and evaluate statistical hypotheses on factors influencing threat perception and exposure. Our results shed light on real-world attacks on deployed machine learning. On the organizational level, while we find no predictors for threat exposure in our sample, the amount of implement defenses depends on exposure to threats or expected likelihood to become a target. We also provide a detailed analysis of practitioners' replies on the relevance of individual machine learning attacks, unveiling complex concerns like unreliable decision making, business information leakage, and bias introduction into models. Finally, we find that on the individual level, prior knowledge about machine learning security influences threat perception. Our work paves the way for more research about adversarial machine learning in practice, but yields also insights for regulation and auditing.

==> IEEEtran/codingtable.tex <==
\begin{table*}[h]
    \centering
        \caption{Inter-coder agreement of free text replies. We compute Spearman correlation ($^*$) and Cohens Kappa ($^\dagger$) for the most feared threat (first question) and the replies of high/low relevance of the five investigated threats. The amount of total codes is the maximum number of codes given from one of the two coders. }\label{tab:interratorAgreement}
    \begin{tabular}{lrrrrrrrrrrrr}
    \toprule
    & & & \multicolumn{2}{c}{Poisoning} & \multicolumn{2}{c}{Evasion} & \multicolumn{2}{c}{Backdoor} & \multicolumn{2}{c}{Membership} & \multicolumn{2}{c}{M. Stealing}
    \\
    \cmidrule(r){4-5}\cmidrule(r){6-7}\cmidrule(r){8-9}\cmidrule(r){10-11}\cmidrule(r){12-13}
     & AML concerns && high & low & high & low & high & low & high & low & high & low \\
    \midrule
    Agreement & $.96^*$ && $.79^\dagger$ &  $.65^\dagger$ &  $.77^\dagger$ & $.69^\dagger$ & $.74^\dagger$ & $.55^\dagger$ & $.67^\dagger$ & $.53^\dagger$ & $.62^\dagger$ & $.55^\dagger$ \\
   \addlinespace
    Total codes & 232 && 86 & 61 & 67 & 63 & 47 & 57 & 54 & 47& 53 & 47 \\
    \# disagreeing & 37 && 6 & 8 & 7 & 8  & 7 & 10 & 8 & 11 & 10 & 9 \\
    \# uncoded & - && 2 & 2 & 3 & - & 4 & 4 & 2 & 4 & 4 & 1 \\
    \# replies & 136 && 69 & 51 & 54 & 49 & 43 & 49 & 45 & 45 & 45 & 40 \\
    \bottomrule
    \end{tabular}
\end{table*}

==> appTests.tex <==

We here report the detailed results for all statistical tests in the main paper in the order of appearance or mentioning.

\subsection{Statistical tests from Section~\ref{sec:orgaStatTests}}
We first review the tests from Section~\ref{sec:orgaStatTests} about the participant's organization in the order of the paragraphs in the main paper.

 
\myparagraph{Organization Area and threat perception} In this part, we depict the detailed results of the organization area and threat relevance ratings. The table takes organizational area (\question{19}), and splits according to Healthcare / Security the provided rating (e.g., participants working in a healthcare setting vs all other participants). We depict mean ($\pm$ standard deviation) and the sample size for each subgroup (left/sample I: works in specified industry, right/sample II: remaining participants) as well as the test statistic and the $p$-value.
\\\begin{tabular}{lrrrrr} \\ 
 \toprule 
 \multicolumn{2}{l}{Sample I} & \multicolumn{2}{l}{Sample II} \\
 \cmidrule(r){1-2} \cmidrule(r){3-4}
 $\mu$ ($\pm $sdt.) & \# &  $\mu$ ($\pm $sdt.) & \# & U & $p$ \\
 \midrule
\multicolumn{4}{l}{Healthcare: Membership Rating (\question{13})} \\ 
1.67 ($\pm$ 1.49) & 18 & 1.71 ($\pm$ 1.85) & 121 & 1030.0 & 0.71 \\ 
 \addlinespace \multicolumn{4}{l}{Security: Poisoning Rating (\question{5})} \\ 
3.0 ($\pm$ 0.97) & 15 & 2.3 ($\pm$ 1.38) & 124 & 1200.0 & 0.06 \\ 
 \addlinespace \multicolumn{4}{l}{Security: Evasion Rating (\question{7})} \\ 
2.73 ($\pm$ 1.44) & 15 & 1.9 ($\pm$ 1.61) & 124 & 1262.0 & \textbf{0.02} \\ 
 \addlinespace \multicolumn{4}{l}{Security: Backdoor Rating (\question{9})} \\ 
3.0 ($\pm$ 0.97) & 15 & 1.6 ($\pm$ 1.74) & 124 & 1372.5 & \textbf{0.0} \\ 
 \addlinespace \multicolumn{4}{l}{Security: Sanity Rating (\question{11})} \\ 
0.4 ($\pm$ 2.06) & 15 & 0.24 ($\pm$ 1.82) & 124 & 953.0 & 0.88 \\ 
 \addlinespace \multicolumn{4}{l}{Security: Membership Rating (\question{13})} \\ 
2.6 ($\pm$ 1.5) & 15 & 1.6 ($\pm$ 1.81) & 124 & 1251.5 & \textbf{0.03} \\ 
 \addlinespace \multicolumn{4}{l}{Security: M. Stealing Rating (\question{15})} \\ 
2.13 ($\pm$ 1.5) & 15 & 1.65 ($\pm$ 1.81) & 124 & 1047.0 & 0.42 \\ 
\bottomrule \end{tabular}

 \myparagraph{Predicting threat exposure} Analogous to the previous tests, we again divide according to company area (\question{19}) and now test for exposure.
  \vspace{0.5em}
 \begin{tabular}{lrrrrr} \\ 
 \toprule
  \multicolumn{2}{l}{Sample I} & \multicolumn{2}{l}{Sample II} \\
 \cmidrule(r){1-2} \cmidrule(r){3-4}
 $\mu$ ($\pm $sdt.) & \# &  $\mu$ ($\pm $sdt.) & \# & U & $p$ \\
 \midrule
\multicolumn{4}{l}{Security: exposure (\question{2})} \\ 
0.44 ($\pm$ 1.21) & 18 & 0.51 ($\pm$ 1.32) & 121 & 1079.0 & 0.93 \\ 
 \addlinespace \multicolumn{4}{l}{Healthcare: exposure (\question{2})} \\ 
1.0 ($\pm$ 1.86) & 15 & 0.44 ($\pm$ 1.21) & 124 & 1038.5 & 0.27 \\ 
 \bottomrule \end{tabular}
  \vspace{0.5em}
  
 We furthermore ran a regression model optimized with bfgs, with the predictors AI maturity (\question{24}) and company size (\question{18}). The obtained log-likelihood of the model was $-96.907$, the AIC $207.8$ and the BIC $228.4$. The model had 132 residuals and 7 degrees of freedom.
 
 \vspace{0.5em}
 
\hspace{-0.5em}
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
                 & coef & std err & z & P$> |$z$|$ & [0.025 & 0.975]  \\
\midrule
AI maturity      &       0.1  &        0.074     &     1.33  &         0.19        &       -0.05    &        0.24     \\
Comp. size      &       0.01  &        0.061     &     0.13  &         0.9        &       -0.11    &        0.13     \\
0.0/1.0 &       1.36  &        0.374     &     3.64  &         0.0       &        0.63    &        2.09     \\
1.0/2.0 &      -1.5  &        0.364     &    -4.11  &         0.0        &       -2.21    &       -0.78     \\
2.0/3.0 &      -1.38  &        0.393     &    -3.51  &         0.0        &       -2.15    &       -0.61     \\
3.0/4.0 &      -2.97  &        0.991     &    -3  &         0.0        &       -4.91    &       -1.03     \\
4.0/5.0 &      -2.15  &        0.695     &    -3.1  &         0.0        &       -3.52    &       -0.79     \\
\bottomrule
\end{tabular}}

\myparagraph{Predicting amount of implemented mitigations}
 To gain insights on the amount of implemented mitigations, we ran a regression model optimized with bfgs. The predictors were AI maturity (\question{24}), company size (\question{18}), exposure (\question{2}) and estimated risk of exposure (\question{3}). As predicted variable, we determine the number of implemented mitigations (min. 0, maximum 7). The obtained log-likelihood was $-266.99$, the AIC $556$ and the BIC $588.3$. The model had 128 residuals and 11 degrees of freedom.

\hspace{-0.7em}
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
    & coef & std err & z & P$> |$z$|$ & [0.025 & 0.975]  \\
\midrule
AI maturity      &       0.15  &        0.051     &     2.84  &         \textbf{0.00}        &        0.045    &        0.246     \\
Comp. size      &       0.01  &        0.043     &     0.17  &         0.87        &       -0.08    &        0.09     \\
Exposure      &       0.18  &        0.071     &     2.5  &         \textbf{0.01}        &        0.04    &        0.32     \\
Est. risk      &       0.2  &        0.079     &     2.5  &         \textbf{0.01}        &        0.04    &        0.35     \\
0.0/1.0 &      -0.06  &        0.316     &    -0.18  &         0.86        &       -0.68    &        0.56     \\
1.0/2.0 &      -0.57  &        0.211     &    -2.7  &         0.01        &       -0.98    &       -0.15     \\
2.0/3.0 &      -0.57  &        0.179     &    -3.2  &         0.00        &       -0.92    &       -0.22     \\
3.0/4.0 &      -0.68  &        0.180     &    -3.8  &         0.00        &       -1.03    &       -0.32     \\
4.0/5.0 &      -0.91  &        0.220     &    -4.1  &         0.00        &       -1.34    &       -0.47     \\
5.0/6.0 &      -1.02  &        0.273     &    -3.7  &         0.00        &       -1.56    &       -0.49     \\
6.0/7.0 &      -1.24  &        0.362     &    -3.4  &         0.00        &       -1.95    &       -0.53     \\
\bottomrule
\end{tabular}}

 \myparagraph{Comparing attack ratings} As reported in the main paper, the Sanity threat (see App.~\ref{app:questionnaire}) is rated statistically significantly different than the other attacks. We here report the detailed results from the attack vs attack ratings. Here, we use the two samples with the numeric inputs for one attack as one input sample. The statistics ($\mu$,std., number of samples) are reported for each attack. we encode  replies without rating as well. 
 
 In addition to the statistical significance for sanity, we also observe statistical significance for poisoning. We do not report this, as we were not able to randomize the order of the attacks, and we assume this is an effect of our participants getting tired. An alternative explanation is that as reported by Kumar et al.~\cite{kumar2020adversarial}, poisoning is indeed the most feared threat (and thus rated higher then other attacks). In addition, the test statistic is also higher when testing against santity for any attack, showing that this effect is stronger.
  \vspace{0.5em}
  
 \hspace{-0.5em}
 \begin{tabular}{lrrrrr} 
 \toprule
  \multicolumn{2}{l}{Attack I} & \multicolumn{2}{l}{Attack II} \\
 \cmidrule(r){1-2} \cmidrule(r){3-4}
 $\mu$ ($\pm $sdt.) & \# &  $\mu$ ($\pm $sdt.) & \# & U & $p$ \\
 \midrule
\multicolumn{2}{l}{Poisoning  (\question{5})} & \multicolumn{2}{l}{Evasion  (\question{7})} \\ 
2.37 ($\pm$ 1.36) & 139 & 1.99 ($\pm$ 1.61) & 139 & 10908 & 0.05 \\ 
 \addlinespace \multicolumn{2}{l}{Poisoning  (\question{5})} & \multicolumn{2}{l}{Backdoor  (\question{9})} \\ 
2.37 ($\pm$ 1.36) & 139 & 1.76 ($\pm$ 1.73) & 139 & 11557 & \textbf{0.0} \\ 
 \addlinespace \multicolumn{2}{l}{Poisoning  (\question{5})} & \multicolumn{2}{l}{Sanity  (\question{11})} \\ 
2.37 ($\pm$ 1.36) & 139 & 0.26 ($\pm$ 1.85) & 139 & 15796 & \textbf{0.0} \\ 
 \addlinespace \multicolumn{2}{l}{Poisoning  (\question{5})} & \multicolumn{2}{l}{Membership  (\question{13})} \\ 
2.37 ($\pm$ 1.36) & 139 & 1.71 ($\pm$ 1.81) & 139 & 11622 & \textbf{0.0} \\ 
 \addlinespace \multicolumn{2}{l}{Poisoning  (\question{5})} & \multicolumn{2}{l}{M. Stealing  (\question{15})} \\ 
2.37 ($\pm$ 1.36) & 139 & 1.71 ($\pm$ 1.79) & 139 & 11566 & \textbf{0.0} \\ 
 \addlinespace \multicolumn{2}{l}{Evasion  (\question{7})} & \multicolumn{2}{l}{Backdoor  (\question{9})} \\ 
1.99 ($\pm$ 1.61) & 139 & 1.76 ($\pm$ 1.73) & 139 & 10327 & 0.31 \\ 
 \addlinespace \multicolumn{2}{l}{Evasion  (\question{7})} & \multicolumn{2}{l}{Sanity  (\question{11})} \\ 
1.99 ($\pm$ 1.61) & 139 & 0.26 ($\pm$ 1.85) & 139 & 14669 & \textbf{0.0} \\ 
 \addlinespace \multicolumn{2}{l}{Evasion  (\question{7})} & \multicolumn{2}{l}{Membership  (\question{13})} \\ 
1.99 ($\pm$ 1.61) & 139 & 1.71 ($\pm$ 1.81) & 139 & 10441 & 0.23 \\ 
 \addlinespace \multicolumn{2}{l}{Evasion  (\question{7})} & \multicolumn{2}{l}{M. Stealing  (\question{15})} \\ 
1.99 ($\pm$ 1.61) & 139 & 1.71 ($\pm$ 1.79) & 139 & 10383 & 0.27 \\ 
 \addlinespace \multicolumn{2}{l}{Backdoor  (\question{9})} & \multicolumn{2}{l}{Sanity  (\question{11})} \\ 
1.76 ($\pm$ 1.73) & 139 & 0.26 ($\pm$ 1.85) & 139 & 14065 & \textbf{0.0} \\ 
 \addlinespace \multicolumn{2}{l}{Backdoor  (\question{9})} & \multicolumn{2}{l}{Membership  (\question{13})} \\ 
1.76 ($\pm$ 1.73) & 139 & 1.71 ($\pm$ 1.81) & 139 & 9789 & 0.84 \\ 
 \addlinespace \multicolumn{2}{l}{Backdoor  (\question{9})} & \multicolumn{2}{l}{M. Stealing  (\question{15})} \\ 
1.76 ($\pm$ 1.73) & 139 & 1.71 ($\pm$ 1.79) & 139 & 9728 & 0.92 \\ 
 \addlinespace \multicolumn{2}{l}{Sanity  (\question{11})} & \multicolumn{2}{l}{Membership  (\question{13})} \\ 
0.26 ($\pm$ 1.85) & 139 & 1.71 ($\pm$ 1.81) & 139 & 5551 & \textbf{0.0} \\ 
 \addlinespace \multicolumn{2}{l}{Sanity  (\question{11})} & \multicolumn{2}{l}{M. Stealing  (\question{15})} \\ 
0.26 ($\pm$ 1.85) & 139 & 1.71 ($\pm$ 1.79) & 139 & 5420 & \textbf{0.0} \\ 
 \addlinespace \multicolumn{2}{l}{Membership  (\question{13})} & \multicolumn{2}{l}{M. Stealing  (\question{15})} \\ 
1.71 ($\pm$ 1.81) & 139 & 1.71 ($\pm$ 1.79) & 139 & 9616 & 0.95 \\ 
\bottomrule 
\end{tabular}


 

\subsection{Statistical tests from Section~\ref{sec:practitioners}}
We first consider the results from Section~\ref{sec:practitioners} about our participants  as in the order of the paragraphs in the main paper.

\textbf{Role in team}
We now split our data according to whether a participant has a technical role (left side) or not (right side).  
\begin{tabular}{lrrrrr} \\
 \toprule 
   \multicolumn{2}{l}{Non-technical} & \multicolumn{2}{l}{Technical} \\
 \cmidrule(r){1-2} \cmidrule(r){3-4}
 $\mu$ ($\pm $sdt.) & \# &  $\mu$ ($\pm $sdt.) & \# & U & $p$ \\
 \midrule
\multicolumn{4}{l}{Exposure (\question{2})} \\ 
0.34 ($\pm$ 1.02) & 91 & 0.81 ($\pm$ 1.68) & 48 & 1970 & 0.15 \\ 
 \addlinespace \multicolumn{4}{l}{Poisoning Rating (\question{5})} \\ 
2.46 ($\pm$ 1.26) & 91 & 2.21 ($\pm$ 1.51) & 48 & 2370 & 0.39 \\ 
 \addlinespace \multicolumn{4}{l}{Evasion Rating (\question{7})} \\ 
1.92 ($\pm$ 1.7) & 91 & 2.12 ($\pm$ 1.41) & 48 & 2135 & 0.83 \\ 
 \addlinespace \multicolumn{4}{l}{Backdoor Rating (\question{9})} \\ 
1.79 ($\pm$ 1.7) & 91 & 1.69 ($\pm$ 1.77) & 48 & 2290 & 0.63 \\ 
 \addlinespace \multicolumn{4}{l}{Sanity Rating (\question{11})} \\ 
0.03 ($\pm$ 1.78) & 91 & 0.69 ($\pm$ 1.92) & 48 & 1756 & 0.05 \\ 
 \addlinespace \multicolumn{4}{l}{Membership Rating (\question{13})} \\ 
1.73 ($\pm$ 1.74) & 91 & 1.67 ($\pm$ 1.93) & 48 & 2151 & 0.89 \\ 
 \addlinespace \multicolumn{4}{l}{M. Stealing Rating (\question{15})} \\ 
1.79 ($\pm$ 1.78) & 91 & 1.54 ($\pm$ 1.79) & 48 & 2340 & 0.48 \\ 
 \bottomrule
 \end{tabular}
 \vspace{0.7em}
 
 
 \myparagraph{Prior Knowledge in AML}
 We now divide our sample along the self-reported knowledge of AML (present, Sample I, not present: Sample II). For the security approaches(\question{4}), we encode the replies using the amount of implemented approaches (e.g., 0-7).
 
  \vspace{0.7em}
  
 \begin{tabular}{rlllll}
 \toprule
\multicolumn{2}{l}{Sample I} & \multicolumn{2}{l}{Sample II} \\
 \cmidrule(r){1-2} \cmidrule(r){3-4}
 $\mu$ ($\pm $sdt.) & \# &  $\mu$ ($\pm $sdt.) & \# & U & $p$ \\
 \midrule
\multicolumn{4}{l}{Exposure (\question{2})} \\ 
0.52 ($\pm$ 1.3) & 40 & 0.49 ($\pm$ 1.31) & 99 & 1991 & 0.94 \\ 
 \addlinespace \multicolumn{4}{l}{Security approaches (\question{4})} \\ 
3.45 ($\pm$ 2.02) & 40 & 2.72 ($\pm$ 2.05) & 99 & 2403 & \textbf{0.05} \\ 
 \addlinespace \multicolumn{4}{l}{Estimated Risk (\question{3})} \\ 
5.5 ($\pm$ 2.26) & 40 & 4.93 ($\pm$ 2.35) & 99 & 2227 & 0.25 \\ 
 \addlinespace \multicolumn{4}{l}{Poisoning Rating (\question{5})} \\ 
2.88 ($\pm$ 0.95) & 40 & 2.17 ($\pm$ 1.44) & 99 & 2533 & \textbf{0.01} \\ 
 \addlinespace \multicolumn{4}{l}{Evasion Rating (\question{7})} \\ 
2.65 ($\pm$ 1.22) & 40 & 1.73 ($\pm$ 1.67) & 99 & 2580 & \textbf{0.0} \\ 
 \addlinespace \multicolumn{4}{l}{Backdoor Rating (\question{9})} \\ 
2.38 ($\pm$ 1.58) & 40 & 1.51 ($\pm$ 1.72) & 99 & 2567 & \textbf{0.01} \\ 
 \addlinespace \multicolumn{4}{l}{Sanity Rating (\question{11})} \\ 
0.52 ($\pm$ 1.96) & 40 & 0.15 ($\pm$ 1.79) & 99 & 2183 & 0.33 \\ 
 \addlinespace \multicolumn{4}{l}{Membership Rating (\question{13})} \\ 
2.4 ($\pm$ 1.51) & 40 & 1.42 ($\pm$ 1.84) & 99 & 2581 & \textbf{0.0} \\ 
 \addlinespace \multicolumn{4}{l}{M. Stealing Rating (\question{15})} \\ 
2.35 ($\pm$ 1.28) & 40 & 1.44 ($\pm$ 1.89) & 99 & 2460 & \textbf{0.02} \\ 
 \bottomrule \end{tabular}
 
\myparagraph{ML knowledge and education}
 We now divide our sample along the self-reported knowledge of ML (present, Sample I, not present: Sample II). For the security approaches(\question{4}), we encode the replies using the amount of implemented approaches (e.g., 0-7).
 \begin{tabular}{lrrrrr} \\ 
 \toprule 
 \multicolumn{2}{l}{Sample I} & \multicolumn{2}{l}{Sample II} \\
 \cmidrule(r){1-2} \cmidrule(r){3-4}
 $\mu$ ($\pm $sdt.) & \# &  $\mu$ ($\pm $sdt.) & \# & U & $p$ \\
 \midrule
\multicolumn{4}{l}{Poisoning Relevance (\question{5})} \\ 
2.55 ($\pm$ 1.08) & 114 & 1.56 ($\pm$ 2.04) & 25 & 1738.0 & 0.07 \\ 
 \addlinespace \multicolumn{4}{l}{Evasion Relevance (\question{7})} \\ 
2.16 ($\pm$ 1.49) & 114 & 1.24 ($\pm$ 1.9) & 25 & 1811.0 & \textbf{0.03} \\ 
 \addlinespace \multicolumn{4}{l}{Backdoor Relevance (\question{9})} \\ 
1.88 ($\pm$ 1.64) & 114 & 1.2 ($\pm$ 1.96) & 25 & 1685.0 & 0.15 \\ 
 \addlinespace \multicolumn{4}{l}{Sanity Relevance (\question{11})} \\ 
0.27 ($\pm$ 1.83) & 114 & 0.2 ($\pm$ 1.96) & 25 & 1480.0 & 0.76 \\ 
 \addlinespace \multicolumn{4}{l}{Membership Relevance (\question{13})} \\ 
1.87 ($\pm$ 1.74) & 114 & 0.96 ($\pm$ 1.93) & 25 & 1811.5 & \textbf{0.03} \\ 
 \addlinespace \multicolumn{4}{l}{Model Stealing Relevance (\question{15})} \\ 
1.85 ($\pm$ 1.71) & 114 & 1.04 ($\pm$ 1.97) & 25 & 1769.5 & 0.05 \\ 
\bottomrule \end{tabular}

 To gain insights on the influence of education, we ran a regression model optimized with bfgs. The predictor was education (\question{29}), the predicted variable exposure (\question{2}). The obtained log-likelihood was $-96.77$, the AIC $205.5$ and the BIC $223.1$. The model had 133 residuals and 6 degrees of freedom.
 
 \vspace{0.5em}
 
 \hspace{-0.7em}
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
                 & coef & std err & z & P$> |$z$|$ & [0.025 & 0.975]  \\
\midrule
Education  &    0.133  &        0.096     &     1.38  &         0.17        &       -0.06    &        0.32     \\
0.0/1.0 &       1.447  &        0.395     &     3.66  &         0.00        &        0.67    &        2.22     \\
1.0/2.0 &      -1.5  &        0.364     &    -4.12  &         0.00        &       -2.22    &       -0.79     \\
2.0/3.0 &      -1.373  &        0.393     &    -3.49  &         0.00        &       -2.14    &       -0.6     \\
3.0/4.0 &      -2.956  &        0.991     &    -2.98  &         0.00        &       -4.9    &       -1.01     \\
4.0/5.0 &      -2.147  &        0.694     &    -3.09  &         0.00        &       -3.51    &       -0.79     \\
\bottomrule
\end{tabular}}

\vspace{0.5em}

We used an analogous model to test the influence of education on estimated risk. The obtained log-likelihood was $-210.71$, the AIC $433.4$ and the BIC $451$. The model had 133 residuals and 6 degrees of freedom.

\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
                  & coef & std err & z & P$> |$z$|$ & [0.025 & 0.975]  \\
\midrule
Education &      0.046  &        0.057     &     0.81  &         0.42        &       -0.07    &        0.16     \\
-1.0/1.0 &      -2.023  &        0.342     &    -5.91  &         0.00        &       -2.69    &       -1.35     \\
1.0/2.0  &       0.321  &        0.199     &     1.61  &         0.11        &       -0.07    &        0.71     \\
2.0/3.0  &      -0.175  &        0.135     &    -1.29  &         0.2        &       -0.44    &        0.09     \\
3.0/4.0  &      -0.086  &        0.132     &    -0.65  &         0.51        &       -0.34    &        0.17     \\
4.0/5.0  &      -0.452  &        0.234     &    -1.93  &         0.05        &       -0.91    &        0.01     \\
\bottomrule
\end{tabular}}
 
 \vspace{2em}
 \myparagraph{Gender} In this section, we divided the sample into female (left) and male (right) participants.
 
 \begin{tabular}{lrrrrr} \\ 
 \toprule 
  \multicolumn{2}{l}{Female} & \multicolumn{2}{l}{Male} \\
 \cmidrule(r){1-2} \cmidrule(r){3-4}
 $\mu$ ($\pm $sdt.) & \# &  $\mu$ ($\pm $sdt.) & \# & U & $p$ \\
 \midrule 
\multicolumn{4}{l}{Estimated Risk (\question{3})} \\ 
2.7 ($\pm$ 0.95) & 20 & 2.46 ($\pm$ 1.26) & 99 & 1098 & 0.43 \\ 
 \addlinespace \multicolumn{4}{l}{exposure (\question{2})} \\ 
0.4 ($\pm$ 1.16) & 20 & 0.6 ($\pm$ 1.43) & 99 & 945 & 0.64 \\ 
 \addlinespace \multicolumn{4}{l}{Poisoning Rating (\question{5})} \\ 
2.1 ($\pm$ 1.34) & 20 & 2.48 ($\pm$ 1.24) & 99 & 846 & 0.28 \\ 
 \addlinespace \multicolumn{4}{l}{Evasion Rating (\question{7})} \\ 
1.65 ($\pm$ 1.53) & 20 & 2.11 ($\pm$ 1.59) & 99 & 811 & 0.19 \\ 
 \addlinespace \multicolumn{4}{l}{Backdoor Rating (\question{9})} \\ 
0.55 ($\pm$ 1.63) & 20 & 1.99 ($\pm$ 1.62) & 99 & 517 & \textbf{0.0} \\ 
 \addlinespace \multicolumn{4}{l}{Sanity Rating (\question{11})} \\ 
-0.15 ($\pm$ 1.53) & 20 & 0.31 ($\pm$ 1.91) & 99 & 867 & 0.37 \\ 
 \addlinespace \multicolumn{4}{l}{Membership Rating (\question{13})} \\ 
1.25 ($\pm$ 1.76) & 20 & 1.83 ($\pm$ 1.79) & 99 & 793 & 0.16 \\ 
 \addlinespace \multicolumn{4}{l}{M. Stealing Rating (\question{15})} \\ 
0.85 ($\pm$ 1.96) & 20 & 1.94 ($\pm$ 1.72) & 99 & 673 & \textbf{0.02} \\ 
 \bottomrule
 \end{tabular}
 

==> codingtable.tex <==
\begin{table*}[h]
    \centering
        \caption{Inter-coder agreement of free text replies. We compute Spearman correlation ($^*$) and Cohens Kappa ($^\dagger$) for the most feared threat (first question) and the replies of high/low relevance of the five investigated threats. The amount of total codes is the maximum number of codes given from one of the two coders. }\label{tab:interratorAgreement}
    \begin{tabular}{lrrrrrrrrrrrr}
    \toprule
    & & & \multicolumn{2}{c}{Poisoning} & \multicolumn{2}{c}{Evasion} & \multicolumn{2}{c}{Backdoor} & \multicolumn{2}{c}{Membership} & \multicolumn{2}{c}{M. Stealing}
    \\
    \cmidrule(r){4-5}\cmidrule(r){6-7}\cmidrule(r){8-9}\cmidrule(r){10-11}\cmidrule(r){12-13}
     & AML concerns && high & low & high & low & high & low & high & low & high & low \\
    \midrule
    Agreement & $.96^*$ && $.79^\dagger$ &  $.65^\dagger$ &  $.77^\dagger$ & $.69^\dagger$ & $.74^\dagger$ & $.55^\dagger$ & $.67^\dagger$ & $.53^\dagger$ & $.62^\dagger$ & $.55^\dagger$ \\
   \addlinespace
    Total codes & 232 && 86 & 61 & 67 & 63 & 47 & 57 & 54 & 47& 53 & 47 \\
    \# disagreeing & 37 && 6 & 8 & 7 & 8  & 7 & 10 & 8 & 11 & 10 & 9 \\
    \# uncoded & - && 2 & 2 & 3 & - & 4 & 4 & 2 & 4 & 4 & 1 \\
    \# replies & 136 && 69 & 51 & 54 & 49 & 43 & 49 & 45 & 45 & 45 & 40 \\
    \bottomrule
    \end{tabular}
\end{table*}

==> codingtableT.tex <==
\begin{table}[]
\centering
\caption{Inter-coder agreement of text replies. We compute Spearman correlation ($^*$) and Cohens Kappa ($^\dagger$) for the most feared threat (\question{1}) and the replies of high/low relevance of the four investigated AML attacks. Total codes refers to the maximum number of codes given from either coder. }\label{tab:interratorAgreement}
\begin{tabular}{llrrrrr}
\toprule
% &  & \rotvertical{Agreement} & \rotvertical{Total}\rotvertical{codes} & \rotvertical{\# disagreeing} & \rotvertical{\# uncoded} & \rotvertical{\# replies} \\  
 
 %&& \rotatebox{72}{Agreement} & \rotatebox{72}{Total codes} & \rotatebox{72}{\# disagreeing} & \rotatebox{72}{\# uncoded} & \rotatebox{72}{\# replies} \\
 &&& Agree- & Total  & \# dis-  & \\
 &&& ment & codes & agreeing  & \# replies \\
 \midrule
 \question{1} & \multicolumn{2}{r}{Most feared threat} & $.96^*$ & 232 & 37  & 136 \\  
 \specialrule{0.25pt}{0.5pt}{0.5pt}
 && high & $.79^\dagger$ & 86 & 6  & 69 \\ 
\multirow{-2}{*}{\question{8}} & \multirow{-2}{*}{Poisoning} & low &
$.65^\dagger$ & 61 & 8  & 51 \\ 
 \addlinespace
 && high & $.77^\dagger$ & 67 & 7 & 54 \\ 
\multirow{-2}{*}{\question{10}}&\multirow{-2}{*}{Evasion} & low & $.69^\dagger$ & 63 & 8  & 49 \\ 
% \addlinespace
%& & high & $.74^\dagger$ & 47 & 7  & 43 \\ 
%\multirow{-2}{*}{\question{12}}&\multirow{-2}{*}{Backdoor} & low & $.55^\dagger$ & 57 & 10  & 49 \\ 
\addlinespace
& & high & $.67^\dagger$ & 54 & 8  & 45 \\ 
\multirow{-2}{*}{\question{16}}&\multirow{-2}{*}{Membership} & low & $.53^\dagger$ & 47 & 11 & 45 \\  
\addlinespace
 && high & $.62^\dagger$ & 53 & 10  & 45 \\ 
\multirow{-2}{*}{\question{18}}&\multirow{-2}{*}{M. Stealing} & low & $.55^\dagger$ & 47 & 9   & 40 \\ \bottomrule
\end{tabular}
\end{table}

==> relevanceTable2.tex <==
%{\rotvertical{Indiscriminate}}}  & \multicolumn{1}{l}{\multirow{3}{*}{\ref{sec:trainingDataSanitization}
%\rdelim\{{3}{*}

\begin{table}[]
\caption{Participants' argumentation for the relevance of attacks. For each attack we present the five most frequent 
(ties broken randomly) arguments (and their frequency).}\label{tab:relevanceCoding}
\begin{tabular}{@{}lrl@{}}
\toprule
  &   \textbf{RELEVANCE} & \textbf{IRRELEVANCE}  \\
%  \cmidrule(r){2-2} \cmidrule(r){3-3}
%  &  Relevance & Irrelevance  \\
  \cmidrule(r){2-2} \cmidrule(r){3-3}
  {\multirow{5}{*}{\rotvertical{Poisoning}}} %\rdelim\{{5}{}
%{\multirow{5}{*}{\textbf{Poisoning}}} \rdelim\{{5}{0.1mm}
  &  \fontfamily{cmss}{Relevant in application (10)}  & \fontfamily{cmss}{(14) No data access}\\
  & \fontfamily{cmss}{Impact on safety (9)} & \fontfamily{cmss}{(9) Not relevant in application}  \\
   & \fontfamily{cmss}{Impact on performance (9)} & \fontfamily{cmss}{(8) Doubting attacker}  \\
  & \fontfamily{cmss}{Relevance without argument (9)} & \fontfamily{cmss}{(5) Human in the loop defense}  \\
  & \fontfamily{cmss}{Hard to defend (7)} & \fontfamily{cmss}{(5) Some defense implemented}  \\
\addlinespace \cmidrule(r){2-2} \cmidrule(r){3-3}
  {\multirow{5}{*}{\rotvertical{Evasion}}}& \fontfamily{cmss}{Impact on model performance (11)}&\fontfamily{cmss}{(11) No data access}  \\
  & \fontfamily{cmss}{Impact on safety (6)} & \fontfamily{cmss}{(10) Not relevant in use case}  \\
   & \fontfamily{cmss}{Impact on decision making (4)} & \fontfamily{cmss}{(7) Doubting attacker}  \\
  &\fontfamily{cmss}{ Easy to do (4)} & \fontfamily{cmss}{(4) Some defense implemented} \\
  & \fontfamily{cmss}{Hard to defend (4)} & \fontfamily{cmss}{(3) Hard to do}  \\
%\addlinespace \cmidrule(r){2-2} \cmidrule(r){3-3}
%  {\multirow{5}{*}{\rotvertical{Backdoor}}}& \fontfamily{cmss}{Impact on safety (6)} & \fontfamily{cmss}{(14) Doubting attacker}  \\
%  & \fontfamily{cmss}{Impact on fairness (6)} & \fontfamily{cmss}{(12) No data access}  \\
%   & \fontfamily{cmss}{Relevance without argument (3)} & \fontfamily{cmss}{(5) Not relevant in use case}  \\
%  & \fontfamily{cmss}{Hard to defend (3)} & \fontfamily{cmss}{(4) Hard to do}  \\
%  & \fontfamily{cmss}{Impact on model performance (3)} & \fontfamily{cmss}{(3) Other threat more likely}  \\
\addlinespace \cmidrule(r){2-2} \cmidrule(r){3-3}
  {\multirow{5}{*}{\rotvertical{Membership}}} & \fontfamily{cmss}{Data breach (21)} & \fontfamily{cmss}{(10) Not relevant in use case}  \\
  & \fontfamily{cmss}{Relevance without argument (3)} & \fontfamily{cmss}{(9) No sensitive data}  \\
   & \fontfamily{cmss}{Business information leakage (3)} & \fontfamily{cmss}{(4) Irrelevance without argument}  \\
  & \fontfamily{cmss}{Regulatory compliance (3)} & \fontfamily{cmss}{(3) No query access}   \\
  & \fontfamily{cmss}{Relevant in application (3)} & \fontfamily{cmss}{(3) Doubting attacker}  \\
\addlinespace \cmidrule(r){2-2} \cmidrule(r){3-3}
 {\multirow{5}{*}{\rotvertical{M. Stealing}}} & \fontfamily{cmss}{Impact on intellectual property (8)} & \fontfamily{cmss}{(13) Not relevant in use case }  \\
  & \fontfamily{cmss}{General business impact (5)} & \fontfamily{cmss}{(7) No query access}  \\
   & \fontfamily{cmss}{Profit for competitor (5)} & \fontfamily{cmss}{(4) Hard to do}  \\
  & \fontfamily{cmss}{Financial loss (4)} &\fontfamily{cmss}{(3) Doubting attacker}  \\
  & \fontfamily{cmss}{Attacker credible (3)} & \fontfamily{cmss}{(3) Model shortlived} \\
\bottomrule
\end{tabular}
\end{table}

==> resultsTable.tex <==
\begin{table}[]
\centering
\caption{Summary of tested statistical hypothesis and findings. Primary variables are in the columns, and are tested against secondary variables in the rows. A \checkmark denotes that the relationship is statistically significant, if there are brackets, some attacks are statistically significant. X\textcolor{white}{,} means there relationship is not statistically significant and $^*$ denotes results which are not discussed in this paper.}\label{tab:resTable}
\begin{tabular}{lrrrr}
\toprule
 & Estimated & Threat  & Number of  &  Attack\\
 & exposure & exposure & mitigations  & concern \\
 \midrule
 Organizational Area &X$^*$ & X\textcolor{white}{,} &X$^*$ & (\checkmark) \\
 AI maturity &X$^*$ & X\textcolor{white}{,} & \checkmark\textcolor{white}{,} &X$^*$ \\
 Company size &X$^*$ & X\textcolor{white}{,} & X\textcolor{white}{,} &X$^*$ \\
 \addlinespace
 Techn./non techn. & X\textcolor{white}{,} & X\textcolor{white}{,} &X$^*$ & X\textcolor{white}{,} \\
 AML knowledge & X\textcolor{white}{,} & X\textcolor{white}{,} & \checkmark\textcolor{white}{,} & \checkmark\textcolor{white}{,} \\
 ML knowledge & X\textcolor{white}{,} & X\textcolor{white}{,} &X$^*$ & (\checkmark) \\
 \addlinespace
 Estimated Exposure & &X$^*$ & \checkmark\textcolor{white}{,} & (\checkmark) \\
 Threat Exposure &X$^*$ & & \checkmark\textcolor{white}{,} & X\textcolor{white}{,}\\
\bottomrule
\end{tabular}
\end{table}
